Cross-language Sentence Selection via Data Augmentation and Rationale Training

This paper proposes an approach to cross-language sentence selection in a low-resource setting. It uses data augmentation and negative sampling techniques on noisy parallel sentence data to directly learn a cross-lingual embedding-based query relevance model. Results show that this approach performs as well as or better than multiple state-of-the-art machine translation + monolingual retrieval systems trained on the same parallel data. Moreover, when a rationale training secondary objective is applied to encourage the model to match word alignment hints from a phrase-based statistical machine translation model, consistent improvements are seen across three language pairs (English-Somali, English-Swahili and English-Tagalog) over a variety of state-of-the-art baselines.

==> Rebuttal.tex <==
\section{Rebuttal}
\subsection{Reviewer \#1}
%Thank you for reviewing our paper! 

We agree that other measures (e.g. NDCG) might productively be reported.
%YC - rephrase to save space
%We choose MAP because the relevance judgments in our test collections are binary, and MAP is a widely used and well-understood measure for binary relevance judgments. 
MAP is a widely used and well-understood measure for **binary** relevance judgments, which are what we have for our test collections. 
Also, MAP models a use case that we care about, where users start at the top of the list and continue until they have read some number of relevant documents. 

%KM - I've rewritten this. 
%We focus on the direction from high-resource queries to low-resource documents because it enables users to find world opinion on a certain topic. Also, this is the direction where we have test collections available for. The reverse direction is of societal importance as well and an important future direction.

We focus on high-resource queries to low-resource documents because in our use case, English speakers want access to information in documents written in any other language. The challenge is in the recovery of relevance from low resource documents. The reverse direction is of societal importance also and an important future direction. 

%KM Nice! Very clear!
%YC: I rewrite this paragraph to make it shorter. I think the original version repeats many things from the paper, and I think the reviewer has understood these concepts. 
In Section 7, we evaluate whether rationale training does help reduce spurious correlations incorporated by the SECLR model (line 319-324) by analyzing the hubness property (line 689-698). By quantitatively showing that rationale training reduces the hubness of the SECLR model, we verify that rationale training is effective in reducing spurious correlations and explain to some degree the improved performance of SECLR-RT over SECLR. 
%In Section 7, we evaluate whether our rationale training technique does help reduce spurious correlations incorporated by the model. For our SECLR model, we observe that irrelevant word pairs are sometimes learned by the model as relevant due to co-occurrences (line 319-324). Such spurious correlations are often present in cross-lingual word embedding spaces, where a few vectors become hubs (line 689-698). 
%CK: I would suggest the following re-write of the last sentence to emphasize that its an explanation not only of spurious correlations but model performance: KM - good!
%We show that rationale training reduces the hubness of the SECLR model and that this explains to some degree both the improved performance of SECLR-RT over SECLR as well as our qualitative observations of spurious correlations learned by SECLR.
%CK: and then finishing with this sentence:
If the paper is accepted we will use our additional space to better motivate this section.

(192 words)

\subsection{Reviewer \#2}
%Thank you for reviewing our paper! 

%CK: Minor Tweak to first sentence:
%YC: I made a small edit to remove the phrase "for training machine translation systems". I think we should avoid confusion since our approach does not train a MT system. Chris, feel free to revert as you see fit. 
Our paper focuses on low-resource settings where we have no collected query-sentence relevance judgment available for training, only a small and noisy parallel corpus. %for training machine translation systems.
%Our paper focuses on low-resource settings where we have no collected query-sentence relevance judgments available for training. 
Results in Table 4,5 show that our SECLR-RT model outperforms all baselines on all test collections. One natural question we then ask is: will we see the same results if the amount of training data (parallel corpus in our case) available is even 
%CK: third sentence: is even fewer? -> is even smaller?
%fewer
smaller? 
For example, there may be a minimum parallel corpus size threshold below which our methods are less effective than the baselines. 
To answer this question, in Section 6 we simulate settings of further data scarcity by restricting model to access only a subsample of the parallel corpus available. In Figure 1, we show that our SECLR-RT model consistently outperforms all baselines in the simulated settings where 
%even fewer parallel corpus is available 
even smaller parallel corpora are available 
for training. 
This experiment gives more context for the IR practitioner working in a low-resource environment as to which methods might be effective in their situation.
We will normalize the y-axis of Figure 1 if the paper gets accepted. 

(179 words)


\subsection{Reviewer \#3}
%Thank you for reviewing our paper! 

Our task is cross-lingual query-sentence relevance prediction. In Appendix D, we include some examples from the evaluation sets that may be helpful. Most English queries in the evaluation sets are short. 

One straightforward approach is to train a model on a relevance dataset of cross-lingual query-sentence pairs labeled with binary relevance judgments. However, our paper focuses on a low-resource setting where no such relevance dataset is available for training, i.e. we do not have a readily available Train collection of the same format as the evaluation collections Analysis/Dev/Eval.

%KM - I added one phrase (second to last sentence, "we propose a data augmentation approach to.." to this very nice explanation to link it with data augmentation (since the reviewer seems to have missed this). Check that you're OK with this. YC - Yes, that looks good. 
To overcome the low-resource challenge of no training data, we propose to generate synthetic training examples (i.e. cross-lingual query-sentence pairs with binary relevance labels) by augmenting a parallel corpus. Conceptually, a parallel corpus is very different from a query-focused relevance dataset. A parallel corpus entails sentence-level semantic equivalence (whether two sentences have the same meaning), but what we need to build a relevance dataset is semantic inclusiveness (whether the short query phrase is semantically included in the sentence). In order to bridge this gap, we propose a data augmentation approach to extract phrases from the English sentences as queries (Section 3.1). Extracting queries from English sentences is not a form of model formalization, but a way to transform a parallel corpus to a query-focused relevance dataset. We only extract unigram queries to reduce over-fitting (line 235-241).

Here are some data augmentation examples. We use the same notations as in Section 3.1. Let's take a sentence pair from the English-Somali parallel corpus (stopwords removed): $E$=``true president gaas attend meeting copenhagen'', $S$=``ma runbaa madaxweyne gaas baaqday shirka copenhegan''. For every unigram $q$ in $E$, we construct a relevant query-sentence pair by extracting $q$ as a query and $S$ as a relevant sentence. 
%YC - rephrase to save space
%For example, we can set $q$=``meeting'' and generate a positive example (``meeting'', ``ma ... copenhegan'', relevant). 
One positive example would be (``meeting'', ``ma ... copenhegan'', relevant).

%KM the reviewer seems to be concerned that you are just doing negative sampling, nothing novel. Can you add a few words to this to indicate that it is not what he assumes. 
We generate negative training examples by pairing up query $q$ with a low-resource sentence randomly selected from the parallel corpus. Let's use $q$=``meeting'' as an example. Randomly select a sentence pair from the English-Somali parallel corpus (stopwords removed): $E'$=``couples main issues destroy somali families wherever'' and $S'$=``lamaanayaasha qodobada waaweyn ee burburiya qoysaska soomaalida meel joogtaba''. In most cases $q$ will be irrelevant to $S'$, but accidentally this may not be true.
% YC - add to emphasize something novel
We propose to use semantic equivalence from parallel corpora to check whether $q$ is relevant to $S'$:
%YC - remove to save space
%To check whether $q$ is relevant to $S'$, 
it suffices to check whether $q$ is relevant to $E'$ because $E'$ and $S'$ are semantically equivalent. Since $q$ and $E'$ are both in English, checking relevance of $q$ to $E'$ is a simple monolingual task (line 255-262). If $q$ is irrelevant to $E'$, then by transitivity $q$ is irrelevant to $S'$, which gives us a negative training example (``meeting'', ``lamaanayaasha ... joogtaba'', irrelevant). 

Besides data augmentation, we also propose a rationale training technique which effectively reduces spurious correlations by incorporating additional alignment information (Section 3.3). Experiments show that in low-resource settings, models are vulnerable to spurious correlations (line 319-325). Rationale training significantly improves model performance (Table 4, 5) and reduces spurious correlations (Section 7). 

We use two-tailed t-tests for significance tests (Footnote 4)
%YC: rephrase to save space
%Our Analysis/Dev/Eval collections contain 300/300/1300 queries, respectively. The size of the test collections thus warrants t-tests. 
because our test collections are large enough (Table 3). 
%CK: I would ask Doug if he can give some citation for what size is appropriate for t-test in IR
We agree, fastText could also have been used for English. %Using word2vec is merely a design choice.

(529 words)

==> material_systcomb_map.tex <==

\begin{table}[t]
\begin{center}
\begin{tabular}{l  c  c c c}
\toprule
 & \multicolumn{2}{c}{Somali} & \multicolumn{2}{c}{Swahili} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
Method   & T & S & T & S \\
\midrule
PSQ (d) & 15.13 & 13.38 & 25.64 & 18.66\\
Sys. Cmb. &  \textbf{15.83}\textsuperscript{$\dagger$} & \textbf{13.67} & \textbf{26.35}\textsuperscript{$\dagger$} & \textbf{19.46}\textsuperscript{$\dagger$} \\
\bottomrule
\end{tabular}
\caption {Document-level Eval MAP scores. \textsuperscript{$\dagger$} indicates
significance at the $p=0.01$ level.}
\label{tab:systcombmap}
\end{center}
\end{table}
